An Epistemic Strategy Logic (Extended Abstract)

The paper presents an extension of temporal epistemic logic with operators that quantify over strategies. The language also provides a natural way to represent what agents would know were they to be aware of the strategies being used by other agents. Some examples are presented to motivate the framework, and relationships to several variants of alternating temporal epistemic logic are discussed. The computational complexity of model checking the logic is also characterized.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{F. Mogavero, A. Murano, and M.Y. Vardi (Eds.): \\
2nd Workshop on Strategic Reasoning 2014 (SR'14)\\
EPTCS 146, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.146.5}{10.4204/EPTCS.146.5}}
\pdfoutput=1

